Toward a Consistent Framework for High Order Mesh Refinement Schemes in Numerical Relativity

It has now become customary in the field of numerical relativity to couple high order finite difference schemes to mesh refinement algorithms. To this end, different modifications to the standard Berger-Oliger adaptive mesh refinement algorithm have been proposed. In this work we present a fourth order stable mesh refinement scheme with sub-cycling in time for numerical relativity. We do not use buffer zones to deal with refinement boundaries but explicitly specify boundary data for refined grids. We argue that the incompatibility of the standard mesh refinement algorithm with higher order Runge Kutta methods is a manifestation of order reduction phenomena, caused by inconsistent application of boundary data in the refined grids. Our scheme also addresses the problem of spurious reflections that are generated when propagating waves cross mesh refinement boundaries. We introduce a transition zone on refined levels within which the phase velocity of propagating modes is allowed to decelerate in order to smoothly match the phase velocity of coarser grids. We apply the method to test problems involving propagating waves and show a significant reduction in spurious reflections.

==> bbl_file <==
\begin{thebibliography}{10}

\bibitem{Babiuc:2007vr}
M.~Babiuc, S.~Husa, D.~Alic, I.~Hinder, C.~Lechner, et~al.
\newblock {Implementation of standard testbeds for numerical relativity}.
\newblock {\em Class.Quant.Grav.}, 25:125012, 2008 arXiv:0709.3559,  [gr-qc].

\bibitem{Baker:2005xe}
J.~G. Baker and J.~R. van Meter.
\newblock {Reducing reflections from mesh refinement interfaces in numerical
  relativity}.
\newblock {\em Phys.Rev.}, D72:104010, 2005 arXiv:gr-qc/0505100,  [gr-qc].

\bibitem{Baumgarte:1998te}
T.~W. Baumgarte and S.~L. Shapiro.
\newblock {On the numerical integration of Einstein's field equations}.
\newblock {\em Phys.Rev.}, D59:024007, 1999 arXiv:gr-qc/9810065,  [gr-qc].

\bibitem{Bentivegna:2012ei}
E.~Bentivegna and M.~Korzynski.
\newblock {Evolution of a periodic eight-black-hole lattice in numerical
  relativity}.
\newblock {\em Class.Quant.Grav.}, 29:165007, 2012 arXiv:1204.3568,  [gr-qc].

\bibitem{Bentivegna:2013jta}
E.~Bentivegna and M.~Korzynski.
\newblock {Evolution of a family of expanding cubic black-hole lattices in
  numerical relativity}.
\newblock {\em Class.Quant.Grav.}, 30:235008, 2013 arXiv:1306.4055,  [gr-qc].

\bibitem{1989JCoPh..82...64B}
M.~J. {Berger} and P.~{Colella}.
\newblock {Local adaptive mesh refinement for shock hydrodynamics}.
\newblock {\em Journal of Computational Physics}, 82:64--84, May 1989.

\bibitem{1984JCoPh..53..484B}
M.~J. {Berger} and J.~{Oliger}.
\newblock {Adaptive Mesh Refinement for Hyperbolic Partial Differential
  Equations}.
\newblock {\em Journal of Computational Physics}, 53:484, March 1984.

\bibitem{Bruegmann:1996kz}
B.~Bruegmann.
\newblock {Adaptive mesh and geodesically sliced Schwarzschild space-time in
  (3+1)-dimensions}.
\newblock {\em Phys.Rev.}, D54:7361--7372, 1996 arXiv:gr-qc/9608050,  [gr-qc].

\bibitem{Bruegmann:1997uc}
B.~Bruegmann.
\newblock {Binary black hole mergers in 3-d numerical relativity}.
\newblock {\em Int.J.Mod.Phys.}, D8:85, 1999 arXiv:gr-qc/9708035,  [gr-qc].

\bibitem{Brugmann:2008zz}
B.~Bruegmann, J.~A. Gonzalez, M.~Hannam, S.~Husa, U.~Sperhake, et~al.
\newblock {Calibration of Moving Puncture Simulations}.
\newblock {\em Phys.Rev.}, D77:024027, 2008 arXiv:gr-qc/0610128,  [gr-qc].

\bibitem{Bruegmann:2006at}
B.~Bruegmann, J.~A. Gonzalez, M.~Hannam, S.~Husa, U.~Sperhake, et~al.
\newblock {Calibration of Moving Puncture Simulations}.
\newblock {\em Phys.Rev.}, D77:024027, 2008 arXiv:gr-qc/0610128,  [gr-qc].

\bibitem{chiltonThesis}
S.~{Chilton}.
\newblock {\em {A fourth order adaptive mesh refinement solver for Maxwell's
  Equations}}.
\newblock PhD thesis, University of California, Berkeley, 2013.

\bibitem{2004JCoPh.193..398C}
D.-I. {Choi}, J.~{David Brown}, B.~{Imbiriba}, J.~{Centrella}, and
  P.~{MacNeice}.
\newblock {Interface conditions for wave propagation through mesh refinement
  boundaries}.
\newblock {\em Journal of Computational Physics}, 193:398--425, January
  2004arXiv:physics/0307036.

\bibitem{PhysRevLett.70.9}
M.~W. Choptuik.
\newblock Universality and scaling in gravitational collapse of a massless
  scalar field.
\newblock {\em Phys. Rev. Lett.}, 70:9--12, Jan 1993.

\bibitem{Csizmadia:2007zz}
P.~Csizmadia.
\newblock {Fourth order AMR and nonlinear dynamical systems in compactified
  space}.
\newblock {\em Class.Quant.Grav.}, 24:S369--S379, 2007.

\bibitem{Debreu:2008:AAG:1316094.1316376}
L.~Debreu, C.~Vouland, and E.~Blayo.
\newblock Agrif: Adaptive grid refinement in fortran.
\newblock {\em Comput. Geosci.}, 34(1):8--13, January 2008.

\bibitem{Diener:2005tn}
P.~Diener, E.~N. Dorband, E.~Schnetter, and M.~Tiglio.
\newblock {New, efficient, and accurate high order derivative and dissipation
  operators satisfying summation by parts, and applications in
  three-dimensional multi-block evolutions}.
\newblock {\em J.Sci.Comput.}, 32:109--145, 2007 arXiv:gr-qc/0512001,  [gr-qc].

\bibitem{ebert02texturing}
D.~S. Ebert, K.~F. Musgrave, D.~Peachey, K.~Perlin, and S.~Worley.
\newblock {\em Texturing and Modeling: A Procedural Approach}.
\newblock Morgan Kaufmann, 2002.

\bibitem{Hairer2009Book}
E.~Hairer, S.~P. N{\o}rsett, and G.~Wanner.
\newblock {\em {Solving Ordinary Differential Equations I: Nonstiff Problems
  (Springer Series in Computational Mathematics) (v. 1)}}.
\newblock Springer, 2nd edition, December 2009.

\bibitem{2010MWRv..138.2174H}
L.~M. {Harris} and D.~R. {Durran}.
\newblock {An Idealized Comparison of One-Way and Two-Way Grid Nesting}.
\newblock {\em Monthly Weather Review}, 138:2174--2187, June 2010.

\bibitem{Herrmann:2007ex}
F.~Herrmann, I.~Hinder, D.~M. Shoemaker, P.~Laguna, and R.~A. Matzner.
\newblock {Binary Black Holes: Spin Dynamics and Gravitational Recoil}.
\newblock {\em Phys.Rev.}, D76:084032, 2007 arXiv:0706.2541,  [gr-qc].

\bibitem{Husa:2007hp}
S.~Husa, J.~A. Gonzalez, M.~Hannam, B.~Bruegmann, and U.~Sperhake.
\newblock {Reducing phase error in long numerical binary black hole evolutions
  with sixth order finite differencing}.
\newblock {\em Class.Quant.Grav.}, 25:105006, 2008 arXiv:0706.0740,  [gr-qc].

\bibitem{Lehner:2005vc}
L.~Lehner, S.~L. Liebling, and O.~Reula.
\newblock {AMR, stability and higher accuracy}.
\newblock {\em Class.Quant.Grav.}, 23:S421--S446, 2006 arXiv:gr-qc/0510111,
  [gr-qc].

\bibitem{2000CoPhC.126..330M}
P.~{MacNeice}, K.~M. {Olson}, C.~{Mobarry}, R.~{de Fainchtein}, and
  C.~{Packer}.
\newblock {PARAMESH: A parallel adaptive mesh refinement community toolkit}.
\newblock {\em Computer Physics Communications}, 126:330--354, April 2000.

\bibitem{mccorquodale2011high}
P.~McCorquodale and P.~Colella.
\newblock A high-order finite-volume method for hyperbolic conservation laws on
  locally-refined grids.
\newblock {\em Communications in Applied Mathematics and Computational
  Science}, 6:1--25, 2011.

\bibitem{bish_thesis:2014}
B.~{Mongwane}.
\newblock {\em {Problems in Cosmology and Numerical Relativity}}.
\newblock PhD thesis, University of Cape Town, 2014.

\bibitem{2004astro.ph..3044O}
B.~W. {O'Shea}, G.~{Bryan}, J.~{Bordner}, M.~L. {Norman}, T.~{Abel},
  R.~{Harkness}, and A.~{Kritsuk}.
\newblock {Introducing Enzo, an AMR Cosmology Application}.
\newblock {\em ArXiv Astrophysics e-prints}, March 2004arXiv:astro-ph/0403044.

\bibitem{2013ApJ...768..115O}
C.~D. {Ott}, E.~{Abdikamalov}, P.~{M{\"o}sta}, R.~{Haas}, S.~{Drasco}, E.~P.
  {O'Connor}, C.~{Reisswig}, C.~A. {Meakin}, and E.~{Schnetter}.
\newblock {General-relativistic Simulations of Three-dimensional Core-collapse
  Supernovae}.
\newblock {\em Astrophys.J.}, 768:115, May 2013 arXiv:1210.6674,
  [astro-ph.HE].

\bibitem{2009JPhCS.180a2022O}
C.~D. {Ott}, E.~{Schnetter}, A.~{Burrows}, E.~{Livne}, E.~{O'Connor}, and
  F.~{L{\"o}ffler}.
\newblock {Computational models of stellar collapse and core-collapse
  supernovae}.
\newblock {\em Journal of Physics Conference Series}, 180(1):012022, July 2009
  arXiv:0907.4043,  [astro-ph.HE].

\bibitem{2011PhRvD..84j4032P}
V.~{Paschalidis}, Y.~T. {Liu}, Z.~{Etienne}, and S.~L. {Shapiro}.
\newblock {Merger of binary white dwarf-neutron stars: Simulations in full
  general relativity}.
\newblock {\em Phys. Rev. D}, 84(10):104032, November 2011 arXiv:1109.5177,
  [astro-ph.HE].

\bibitem{Pollney:2009yz}
D.~Pollney, C.~Reisswig, E.~Schnetter, N.~Dorband, and P.~Diener.
\newblock {High accuracy binary black hole simulations with an extended wave
  zone}.
\newblock {\em Phys.Rev.}, D83:044045, 2011 arXiv:0910.3803,  [gr-qc].

\bibitem{MohanRai1986472}
M.~M. Rai.
\newblock A conservative treatment of zonal boundaries for euler equation
  calculations.
\newblock {\em Journal of Computational Physics}, 62(2):472 -- 503, 1986.

\bibitem{Roma1999509}
A.~M. Roma, C.~S. Peskin, and M.~J. Berger.
\newblock An adaptive version of the immersed boundary method.
\newblock {\em Journal of Computational Physics}, 153(2):509 -- 534, 1999.

\bibitem{Schnetter:2003rb}
E.~Schnetter, S.~H. Hawley, and I.~Hawke.
\newblock {Evolutions in 3-D numerical relativity using fixed mesh refinement}.
\newblock {\em Class.Quant.Grav.}, 21:1465--1488, 2004 arXiv:gr-qc/0310042,
  [gr-qc].

\bibitem{Shen:2011:AMR:1963655.1963728}
C.~Shen, J.-M. Qiu, and A.~Christlieb.
\newblock Adaptive mesh refinement based on high order finite difference weno
  scheme for multi-scale simulations.
\newblock {\em J. Comput. Phys.}, 230(10):3780--3802, May 2011.

\bibitem{Shibata:1999yx}
M.~Shibata, T.~W. Baumgarte, and S.~L. Shapiro.
\newblock {Stability and collapse of rapidly rotating, supramassive neutron
  stars: 3-D simulations in general relativity}.
\newblock {\em Phys.Rev.}, D61:044012, 2000 arXiv:astro-ph/9911308,
  [astro-ph].

\bibitem{Skamarock01adescription}
W.~C. Skamarock, J.~B. Klemp, J.~Dudhia, D.~O. Gill, D.~M. Barker, W.~Wang, and
  J.~G. Powers.
\newblock A description of the advanced research wrf version 2.
\newblock {\em Available from NCAR; P.O. Box 3000; Boulder, co}, 88:7--25,
  2001.

\bibitem{Takami:2014zpa}
K.~Takami, L.~Rezzolla, and L.~Baiotti.
\newblock {Constraining the Equation of State of Neutron Stars from Binary
  Mergers}.
\newblock {\em Phys.Rev.Lett.}, 113(9):091104, 2014 arXiv:1403.5672,  [gr-qc].

\bibitem{PhysRevD.26.745}
S.~A. Teukolsky.
\newblock Linearized quadrupole waves in general relativity and the motion of
  test particles.
\newblock {\em Phys. Rev. D}, 26:745--750, Aug 1982.

\bibitem{Ziegler2008227}
U.~Ziegler.
\newblock The nirvana code: Parallel computational mhd with adaptive mesh
  refinement.
\newblock {\em Computer Physics Communications}, 179(4):227 -- 244, 2008.

\bibitem{Zilhao:2014wqa}
M.~Zilhão, V.~Cardoso, C.~Herdeiro, L.~Lehner, and U.~Sperhake.
\newblock {Testing the nonlinear stability of Kerr-Newman black holes}.
\newblock {\em Phys.Rev.}, D90:124088, 2014 arXiv:1410.0694,  [gr-qc].

\bibitem{Zlochower:2005bj}
Y.~Zlochower, J.~Baker, M.~Campanelli, and C.~Lousto.
\newblock {Accurate black hole evolutions by fourth-order numerical
  relativity}.
\newblock {\em Phys.Rev.}, D72:024021, 2005 arXiv:gr-qc/0505055,  [gr-qc].

\bibitem{PhysRevD.86.104056}
Y.~Zlochower, M.~Ponce, and C.~O. Lousto.
\newblock Accuracy issues for numerical waveforms.
\newblock {\em Phys. Rev. D}, 86:104056, Nov 2012.

\end{thebibliography}

